REACT: Autonomous Intrusion Response System for Intelligent Vehicles

Autonomous and connected vehicles are rapidly evolving, integrating numerous technologies and software. This progress, however, has made them appealing targets for cybersecurity attacks. As the risk of cyber threats escalates with this advancement, the focus is shifting from solely preventing these attacks to also mitigating their impact. Current solutions rely on vehicle security operation centers, where attack information is analyzed before deciding on a response strategy. However, this process can be time-consuming and faces scalability challenges, along with other issues stemming from vehicle connectivity. This paper proposes a dynamic intrusion response system integrated within the vehicle. This system enables the vehicle to respond to a variety of incidents almost instantly, thereby reducing the need for interaction with the vehicle security operation center. The system offers a comprehensive list of potential responses, a methodology for response evaluation, and various response selection methods. The proposed solution was implemented on an embedded platform. Two distinct cyberattack use cases served as the basis for evaluating the system. The evaluation highlights the system's adaptability, its ability to respond swiftly, its minimal memory footprint, and its capacity for dynamic system parameter adjustments. The proposed solution underscores the necessity and feasibility of incorporating dynamic response mechanisms in smart vehicles. This is a crucial factor in ensuring the safety and resilience of future smart mobility.

==> fig/arch.tex <==
\begin{tikzpicture}
\node[draw,text width=\textwidth, minimum height=0.7*\textwidth] at (0,0) {};

\node[draw,text width=3cm, minimum height=3cm, align=center] at (-0.35*\textwidth,0.2*\textwidth) {\ac{IDS}};

\draw (-0.24*\textwidth,0.2*\textwidth) -- (-0.21*\textwidth,0.2*\textwidth);
\draw (-0.21*\textwidth,0.2*\textwidth) -- (-0.21*\textwidth,0.15*\textwidth);
\draw [-stealth](-0.21*\textwidth,0.15*\textwidth) -- (-0.153*\textwidth,0.15*\textwidth);
\draw [stealth-](-0.46*\textwidth,0.2*\textwidth) -- (-0.52*\textwidth,0.2*\textwidth);
\node[align=left] at (-0.55*\textwidth,0.2*\textwidth){\ac{IDS}\\data};

\node[draw,text width=5cm, minimum height=3cm, align=center] at (0*\textwidth,0.2*\textwidth) {};
\node[text centered] at (0,0.325*\textwidth){Risk Evaluation Module};
\node[draw,text width=2.3cm, minimum height=0.7cm, align=center, fill=lightgray] at (-0.07*\textwidth,0.25*\textwidth) {\small Environmental\\\small Sensing};
\node[draw,text width=1.3cm, minimum height=0.7cm, align=center, fill=lightgray] at (-0.1*\textwidth,0.15*\textwidth) {\small \ac{TARA}};
\node[draw,text width=1.3cm, minimum height=0.7cm, align=center, fill=lightgray] at (0.1*\textwidth,0.15*\textwidth) {\small Policy};
\draw [-stealth](-0.21*\textwidth,0.25*\textwidth) -- (-0.157*\textwidth,0.25*\textwidth);
\draw (-0.21*\textwidth,0.25*\textwidth) -- (-0.21*\textwidth,0.38*\textwidth);
\draw [-stealth](0.046*\textwidth,0.14*\textwidth) -- (-0.047*\textwidth,0.14*\textwidth);
\draw (0.03*\textwidth,0.16*\textwidth) -- (-0.047*\textwidth,0.16*\textwidth);
\draw (0.03*\textwidth,0.25*\textwidth) -- (0.017*\textwidth,0.25*\textwidth);
\draw (0.03*\textwidth,0.25*\textwidth) -- (0.03*\textwidth,0.16*\textwidth);
\node[align=center] at (-0.21*\textwidth,0.39*\textwidth){Vehicle and Environmental Data};

\draw [-stealth](0.03*\textwidth,0.2*\textwidth) -- (0.24*\textwidth,0.2*\textwidth);

\node[draw,text width=3cm, minimum height=3cm, align=center] at (0.35*\textwidth,0.2*\textwidth) {Response Set Generation};

\draw (0.35*\textwidth,0.099*\textwidth) -- (0.35*\textwidth,-0.25*\textwidth);
\draw [-stealth](0.35*\textwidth,-0.25*\textwidth) -- (0.311*\textwidth,-0.25*\textwidth);

\node[draw,text width=3cm, minimum height=2cm, align=center] at (0.2*\textwidth,-0.25*\textwidth) {Optimal\\Response\\Selection};

\draw [-stealth](0.09*\textwidth,-0.25*\textwidth) -- (0.035*\textwidth,-0.25*\textwidth);
\draw [-stealth](0.2*\textwidth,-0.14*\textwidth) -- (0.2*\textwidth,-0.182*\textwidth);
\draw (0.2*\textwidth,-0.14*\textwidth) -- (-0.075*\textwidth,-0.14*\textwidth);
\draw (-0.075*\textwidth,-0.14*\textwidth) -- (-0.075*\textwidth,-0.182*\textwidth);

\node[draw,text width=3cm, minimum height=2cm, align=center] at (-0.075*\textwidth,-0.25*\textwidth) {Precondition Checking};

\draw [-stealth](-0.185*\textwidth,-0.25*\textwidth) -- (-0.24*\textwidth,-0.25*\textwidth);

\node[draw,text width=3cm, minimum height=2cm, align=center] at (-0.35*\textwidth,-0.25*\textwidth) {Response Execution and Delivery};

\draw [-stealth](-0.35*\textwidth,-0.182*\textwidth) -- (-0.35*\textwidth,-0.051*\textwidth);
\draw [-stealth](-0.46*\textwidth,-0.25*\textwidth) -- (-0.52*\textwidth,-0.25*\textwidth);
\node[text centered] at (-0.58*\textwidth,-0.25*\textwidth){Responses};

\node[draw,text width=3cm, minimum height=1.5cm, align=center] at (-0.35*\textwidth,0*\textwidth) {\ac{IDS} Feedback};

\draw [stealth-](-0.35*\textwidth,0.098*\textwidth) -- (-0.35*\textwidth,0.051*\textwidth);
\draw [-stealth](-0.24*\textwidth,0.035*\textwidth) -- (-0.11*\textwidth,0.035*\textwidth);
\draw [-stealth](-0.13*\textwidth,0.035*\textwidth) -- (-0.13*\textwidth,0.125*\textwidth);
\draw [stealth-](-0.46*\textwidth,-0.0*\textwidth) -- (-0.52*\textwidth,-0.0*\textwidth);
\node[align=left] at (-0.58*\textwidth,-0.0*\textwidth){Monitoring\\Feedback};

\node[draw,text width=3cm, minimum height=1.5cm, align=center] at (0*\textwidth,0*\textwidth) {Response Storage};

\draw (-0.11*\textwidth,0.0*\textwidth) -- (-0.205*\textwidth,0.0*\textwidth);
\draw (-0.205*\textwidth,0.0*\textwidth) -- (-0.205*\textwidth,-0.2*\textwidth);
\draw [-stealth](-0.205*\textwidth,-0.2*\textwidth) -- (-0.24*\textwidth,-0.2*\textwidth);
\draw (-0.11*\textwidth,-0.035*\textwidth) -- (-0.15*\textwidth,-0.035*\textwidth);
\draw [-stealth](-0.15*\textwidth,-0.035*\textwidth) -- (-0.15*\textwidth,-0.182*\textwidth);
\draw (0.11*\textwidth,0.035*\textwidth) -- (0.3*\textwidth,0.035*\textwidth);
\draw [-stealth](0.3*\textwidth,0.035*\textwidth) -- (0.3*\textwidth,0.099*\textwidth);
\draw (0.11*\textwidth,-0.035*\textwidth) -- (0.25*\textwidth,-0.035*\textwidth);
\draw [-stealth](0.25*\textwidth,-0.035*\textwidth) -- (0.25*\textwidth,-0.182*\textwidth);

\node[draw,text width=2cm, minimum height=1cm, align=center] at (0.42*\textwidth,-0.3*\textwidth) {(Secure)\\Storage};
\draw [stealth-](0.42*\textwidth,-0.338*\textwidth) -- (0.42*\textwidth,-0.38*\textwidth);
\node[align=center] at (0.42*\textwidth,-0.4*\textwidth){Additional data};

\draw [stealth-stealth](0.21*\textwidth,0.35*\textwidth) -- (0.21*\textwidth,0.38*\textwidth);
\node[align=center] at (0.21*\textwidth,0.39*\textwidth){External connectivity};
\end{tikzpicture}

==> fig/fig-arc.tex <==
\begin{tikzpicture}

\newcommand{\gwheight}{1.5cm}
\newcommand{\gwwidth}{2cm}
\newcommand{\ecuheight}{1cm}

\node[draw,text width=\textwidth, minimum height=\gwheight, align=center] at (0,0) {Central in-vehicle Gateway};

\node[draw,text width=\gwwidth, minimum height=\gwheight, align=center] at (-2.5,2.5) {Diagnostic interface};
\node[draw,text width=\gwwidth, minimum height=\gwheight, align=center] at (0,2.5) {External communication};
\node[draw,text width=\gwwidth, minimum height=\gwheight, align=center] at (-0.5*\textwidth+0.5*\gwwidth,-2.5) {Powertrain};
\node[draw,text width=\gwwidth, minimum height=\gwheight, align=center] at (-0.285*\textwidth+0.5*\gwwidth,-2.5) {Body / Comfort};
\node[draw,text width=\gwwidth, minimum height=\gwheight, align=center] at (0,-2.5) {Chassis};
\node[draw,text width=\gwwidth, minimum height=\gwheight, align=center] at (0.285*\textwidth-0.5*\gwwidth,-2.5) {\acs{ADAS} \small (incl. sensor fusion)};
\node[draw,text width=1.1*\gwwidth, minimum height=\gwheight, align=center] at (0.5*\textwidth-0.5*\gwwidth,-2.5) {Infotainment};

\draw[red] (0,0.5*\gwheight) -- (0,0.5*\gwheight+28);
\draw[red] (-2.5,0.5*\gwheight) -- (-2.5,0.5*\gwheight+28);
\draw[red] (-0.5*\textwidth+0.5*\gwwidth,-0.5*\gwheight) -- (-0.5*\textwidth+0.5*\gwwidth,-0.5*\gwheight-28);
\draw[red] (-0.285*\textwidth+0.5*\gwwidth,-0.5*\gwheight) -- (-0.285*\textwidth+0.5*\gwwidth,-0.5*\gwheight-28);
\draw[red] (0,-0.5*\gwheight) -- (0,-0.5*\gwheight-28);
\draw[red] (0.285*\textwidth-0.5*\gwwidth,-0.5*\gwheight) -- (0.285*\textwidth-0.5*\gwwidth,-0.5*\gwheight-28);
\draw[red] (0.5*\textwidth-0.5*\gwwidth,-0.5*\gwheight) -- (0.5*\textwidth-0.5*\gwwidth,-0.5*\gwheight-28);

\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (-5,3.3) {\small \ac{OBD}-II};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (-5,1.7) {\small \ac{DoIP}};
\draw[black] (-5,2.5) -- (-3.62,2.5);
\draw[black] (-5,2.5) -- (-5,2.8);
\draw[black] (-5,2.5) -- (-5,2.2);

\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (2.5,3.3) {\small \ac{GPS}};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (5,3.3) {\small Cellular module};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (7.5,3.3) {\small \ac{DSRC} for \ac{IoV}};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (2.5,1.7) {\small \acs{EV} charging};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (5,1.7) {\small Digital toll collection};
\draw[black] (1.13,2.5) -- (7.5,2.5);
\draw[black] (2.5,2.2) -- (2.5,2.8);
\draw[black] (5,2.2) -- (5,2.8);
\draw[black] (7.5,2.5) -- (7.5,2.8);

\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+0.5*\gwwidth,-4.2) {\small Engine control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+0.5*\gwwidth,-5.4) {\small Transmission control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+0.5*\gwwidth,-6.6) {\small Battery management};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+0.5*\gwwidth,-7.8) {\small Combustion control};
\draw[green] (-0.5*\textwidth+0.5*\gwwidth,-3.25) -- (-0.5*\textwidth+0.5*\gwwidth,-7.8);
\draw[green] (-0.6*\textwidth+1.07*\gwwidth,-4.2) -- (-0.5*\textwidth+0.5*\gwwidth,-4.2);
\draw[green] (-0.6*\textwidth+1.07*\gwwidth,-5.4) -- (-0.5*\textwidth+0.5*\gwwidth,-5.4);
\draw[green] (-0.6*\textwidth+1.07*\gwwidth,-6.6) -- (-0.5*\textwidth+0.5*\gwwidth,-6.6);
\draw[green] (-0.6*\textwidth+1.07*\gwwidth,-7.8) -- (-0.5*\textwidth+0.5*\gwwidth,-7.8);

\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+2.1*\gwwidth,-4.2) {\small Light control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+2.1*\gwwidth,-5.4) {\small Wiper control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (-0.6*\textwidth+2.1*\gwwidth,-6.6) {\small Key control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+2.1*\gwwidth,-7.8) {\small Climate control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+2.1*\gwwidth,-9) {\small Door/Trunk control};
\draw[violet] (-0.285*\textwidth+0.5*\gwwidth,-3.25) -- (-0.285*\textwidth+0.5*\gwwidth,-9);
\draw[violet] (-0.285*\textwidth+0.5*\gwwidth,-4.2) -- (-0.285*\textwidth+0.35*\gwwidth,-4.2);
\draw[violet] (-0.285*\textwidth+0.5*\gwwidth,-5.4) -- (-0.285*\textwidth+0.35*\gwwidth,-5.4);
\draw[violet] (-0.285*\textwidth+0.5*\gwwidth,-6.6) -- (-0.285*\textwidth+0.35*\gwwidth,-6.6);
\draw[violet] (-0.285*\textwidth+0.5*\gwwidth,-7.8) -- (-0.285*\textwidth+0.35*\gwwidth,-7.8);
\draw[violet] (-0.285*\textwidth+0.5*\gwwidth,-9) -- (-0.285*\textwidth+0.35*\gwwidth,-9);

\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+3.7*\gwwidth,-4.2) {\small Steering control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+3.7*\gwwidth,-5.4) {\small Acceleration control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+3.7*\gwwidth,-6.6) {\small Brake control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+3.7*\gwwidth,-7.8) {\small Airbag control};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+3.7*\gwwidth,-9) {\small Instrument cluster};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (-0.6*\textwidth+3.7*\gwwidth,-10.2) {\small \ac{TPMS} receiver};
\draw[cyan] (0,-3.25) -- (0,-6.6);
\draw[cyan] (0,-4.2) -- (-0.28,-4.2);
\draw[cyan] (0,-5.4) -- (-0.28,-5.4);
\draw[cyan] (0,-6.6) -- (-0.28,-6.6);
\draw[green] (0.28,-3.25) -- (0.28,-10.2);
\draw[green] (0.28,-7.8) -- (-0.28,-7.8);
\draw[green] (0.28,-9) -- (-0.28,-9);
\draw[green] (0.28,-10.2) -- (-0.28,-10.2);

\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+5.3*\gwwidth,-4.2) {\small Front camera(s)};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+5.3*\gwwidth,-5.4) {\small Surround camera(s)};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+5.3*\gwwidth,-6.6) {\small Radar(s)};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+5.3*\gwwidth,-7.8) {\small \acs{LiDAR}};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (-0.6*\textwidth+5.3*\gwwidth,-9) {\small Ultrasonic};
\draw[red] (0.285*\textwidth-0.5*\gwwidth,-3.29) -- (0.285*\textwidth-0.5*\gwwidth,-9);
\draw[red] (0.285*\textwidth-0.5*\gwwidth,-4.2) -- (0.285*\textwidth-0.64*\gwwidth,-4.2);
\draw[red] (0.285*\textwidth-0.5*\gwwidth,-5.4) -- (0.285*\textwidth-0.64*\gwwidth,-5.4);
\draw[red] (0.285*\textwidth-0.5*\gwwidth,-6.6) -- (0.285*\textwidth-0.64*\gwwidth,-6.6);
\draw[red] (0.285*\textwidth-0.5*\gwwidth,-7.8) -- (0.285*\textwidth-0.64*\gwwidth,-7.8);
\draw[red] (0.285*\textwidth-0.5*\gwwidth,-9) -- (0.285*\textwidth-0.64*\gwwidth,-9);

\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (0.5*\textwidth-1.2*\gwwidth,-4.2) {\small WiFi hotspot};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (0.5*\textwidth-1.2*\gwwidth,-5.4) {\small \ac{USB} port(s)};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (0.5*\textwidth-1.2*\gwwidth,-6.6) {\small Video screens};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (0.5*\textwidth-1.2*\gwwidth,-7.8) {\small Bluetooth};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=white] at (0.5*\textwidth-1.2*\gwwidth,-9) {\small Speech recognition};
\node[draw,text width=\gwwidth, minimum height=\ecuheight, align=center, fill=orange] at (0.5*\textwidth-1.2*\gwwidth,-10.2) {\small \acs{FM}/\acs{DAB} Radio};
\draw[red] (0.5*\textwidth-0.5*\gwwidth,-3.25) -- (0.5*\textwidth-0.5*\gwwidth,-10.2);
\draw[red] (0.5*\textwidth-0.5*\gwwidth,-4.2) -- (0.5*\textwidth-0.64*\gwwidth,-4.2);
\draw[red] (0.5*\textwidth-0.5*\gwwidth,-5.4) -- (0.5*\textwidth-0.64*\gwwidth,-5.4);
\draw[red] (0.5*\textwidth-0.5*\gwwidth,-6.6) -- (0.5*\textwidth-0.64*\gwwidth,-6.6);
\draw[red] (0.5*\textwidth-0.5*\gwwidth,-7.8) -- (0.5*\textwidth-0.64*\gwwidth,-7.8);
\draw[red] (0.5*\textwidth-0.5*\gwwidth,-9) -- (0.5*\textwidth-0.64*\gwwidth,-9);
\draw[red] (0.5*\textwidth-0.5*\gwwidth,-10.2) -- (0.5*\textwidth-0.64*\gwwidth,-10.2);

\node[draw,text width=1.1*\gwwidth, minimum height=2*\ecuheight, align=left, fill=white] at (-0.6*\textwidth+0.5*\gwwidth,2.5) {\small \colorbox{cyan}{\textcolor{cyan}{\normalsize \textbf{---}}}=FlexRay\\\colorbox{green}{\textcolor{green}{\normalsize \textbf{---}}}=\acs{CAN}\\\colorbox{violet}{\textcolor{violet}{\normalsize \textbf{---}}}=\acs{LIN}\\\colorbox{red}{\textcolor{red}{\normalsize \textbf{---}}}=Ethernet\\\colorbox{black}{\textcolor{black}{\normalsize \textbf{---}}}=Divers\\\colorbox{orange}{\textcolor{orange}{\normalsize \textbf{---}}}=Source};

\end{tikzpicture}

==> sections/relatedwork.tex <==
\section{Related Work}
\subsection*{automotive IRS}
\subsection*{automotive IRS}
